On Matching and Thickness in Heterogeneous Dynamic Markets

We study dynamic matching in an infinite-horizon stochastic market. While all agents are potentially compatible with each other, some are hard-to-match and others are easy-to-match. Agents prefer to be matched as soon as possible and matches are formed either bilaterally or indirectly through chains. We adopt an asymptotic approach and compute tight bounds on the limit of waiting time of agents under myopic policies that differ in matching technology and prioritization. We find that the market composition is a key factor in the desired matching technology and prioritization level. When hard-to-match agents arrive less frequently than easy-to-match ones (i) bilateral matching is almost as efficient as chains (waiting times scale similarly under both, though chains always outperform bilateral matching by a constant factor), and (ii) assigning priorities to hard-to-match agents improves their waiting times. When hard-to-match agents arrive more frequently, chains are much more efficient than bilateral matching and prioritization has no impact. We further conduct comparative statics on arrival rates. Somewhat surprisingly, we find that in a heterogeneous market and under bilateral matching, increasing arrival rate has a non-monotone effect on waiting times, due to the fact that, under some market compositions, there is an adverse effect of competition. Our comparative statics shed light on the impact of merging markets and attracting altruistic agents (that initiate chains) or easy-to-match agents. This work uncovers fundamental differences between heterogeneous and homogeneous dynamic markets, and potentially helps policy makers to generate insights on the operations of matching markets such as kidney exchange programs.

==> bilateral_proofs.tex <==
%\subsection{Proof idea of Theorem \ref{th:bilat_prioH}}
\subsection{\textit{ BilateralMatch(H)} Policy}
\label{subsec:BH}
Under $\BH$, the evolution of the number of $H$ and $E$ agents in the market can be modeled by a  CTMC $[H_t^{\BH},  E_t^{\BH}] \in \Z^2$ with the following rate matrix:

\begin{subequations}
%\label{eq:transitions}
\begin{align}
Q^{\BH}([h,e],[h+1,e]) &= \lambda_H (1 - p_H^2)^{h} (1 - p_E p_H)^{e} \label{eq:transtion:1}\\
Q^{\BH}([h,e],[h-1,e]) &=  \lambda_H (1 - (1 - p_H^2)^{h}) + \lambda_E (1 - (1 - p_E p_H)^{h}) \label{eq:transtion:2}\\
Q^{\BH}([h,e],[h,e + 1])&=\lambda_E (1 - p_E p_H)^{h} (1 - p_E^2)^{e} \label{eq:transtion:3}\\
Q^{\BH}([h,e],[h,e-1])&= \lambda_H (1 - p_H^2)^{h} (1 - (1 - p_E p_H)^{e}) + \lambda_E (1 - p_E p_H)^{h} (1 - (1 - p_E^2)^{e})) \label{eq:transtion:4}
\end{align}
\end{subequations}

The rates are computed based on the Poisson thinning property, simple counting arguments,  and the fact that a directed edge between the arriving agent and each of the existing agents in the market exists independently.

\begin{itemize}
\item[-]Leftward rate \eqref{eq:transtion:1}: we move from $[h,e]$ to $[h+1,e]$ iff an $H$ agent arrives and cannot form a $2$-way with any of the existing $H$ agents (which happens with probability $(1 - p_H^2)^{h}$), and cannot form a $2$-way with any of the existing $E$ agents either (which happens with probability $(1 - p_E p_H)^{e}$.
\item[-]Rightward rate \eqref{eq:transtion:2}: we move from $[h,e]$ to $[h-1,e]$ iff an $H$ agent arrives and forms a $2$-way with at least one of the existing $H$ agents  (which happens with probability $(1 - (1 - p_H^2)^{h})$) or an $E$ agent arrives and forms a $2$-way with at least one of the existing $H$ agents (which happens with probability $(1 - (1 - p_E p_H)^{h}) $).
\item[-] Upward rate \eqref{eq:transtion:3}: we move from $[h,e]$ to $[h,e+1]$ iff an $E$ agent arrives and cannot form a $2$-way with any of the existing $H$ agents (which happens with probability $(1 - p_E p_H)^{h}$), and cannot form a $2$-way with any of the existing $E$ agents either (which happens with probability $(1 - p_E^2 )^{e}$).
\item[-] Downward rate \eqref{eq:transtion:4}: we move from $[h,e]$ to $[h,e-1]$ iff an $H$ agent arrives that cannot  form a $2$-way with any of the existing $H$ agents (which happens with probability $(1 - p_H^2)^{h}$) but can form a $2$-way with at least one of the existing $E$ agents (which happens with probability $(1 - (1 - p_E p_H)^{e})$), or an $E$ agent arrives that cannot form  form a $2$-way with any of the existing $H$ agents (which happens with probability $(1 - p_Ep_H)^{h}$) but can form a $2$-way with at least one of the existing $E$ agents (which happens with probability $(1 - (1 - p_E^2)^{e})$).
\end{itemize}

%We start by \eqref{eq:transtion:1}: we move from $[h,e]$ to $[h+1,e]$ iff an $H$ agent arrives and cannot form a $2$-way with any of the existing $H$ agents (which happens with probability (1 - p_H^2)^{h}), and cannot form a $2$-way with any of the existing $E$ agents either (which happens with probability $(1 - p_E p_H)^{e}$.



\begin{figure}[htbp]
\centering
\begin{tikzpicture}
[align=center,node distance=1.7cm]
\node[state, minimum size=1.5cm] (s) {\small [h, e]};
\node[state, minimum size=1.5cm, node distance=4.5cm, right=of s] (r) {\small [h+1, e]};
\node[state, minimum size=1.5cm, node distance=4.5cm, left=of s] (l) {\small [h-1, e]};
\node[state, minimum size=1.5cm, node distance=2.5cm, above=of s] (t) {\small [h, e+1]};
\node[state, minimum size=1.5cm, node distance=2.5cm, below=of s] (b) {\small [h, e-1]};
\node[draw=none, minimum size=1.5cm, node distance=4.5cm, right=of b] (br) {...};
\node[draw=none, minimum size=1.5cm, node distance=4.5cm, left=of b] (bl) {...};
\node[draw=none, minimum size=1.5cm, node distance=4.5cm, right=of t] (tr) {...};
\node[draw=none, minimum size=1.5cm, node distance=4.5cm, left=of t] (tl) {...};
        % Connect the states with arrows
        \draw[every loop, line width=0.6mm, >=latex]
%		(s) edge[bend right, auto=left] node {\tiny $Q\left([h,e],[h+1,e]\right)$} (r)
%		(r) edge[bend right] node {} (s)
%		(s) edge[bend right, auto=left] node {\tiny $Q([h,e],[h-1,e])$} (l)
%		(l) edge[bend right] node {} (s)
%		(s) edge[bend right, auto=right] node {\tiny $Q([h,e],[h,e + 1])$} (t)
%		(t) edge[bend right] node {} (s)
%		(s) edge[bend right, auto=right] node {\tiny $Q([h,e],[h,e - 1])$} (b)
		(s) edge[bend right,auto=left] node[below] {\scriptsize $\lambda_H (1 - p_H^2)^{h} (1 - p_E p_H)^{e}$} (r)
		(r) edge[bend right, dashed] node {} (s)
		(s) edge[bend right, auto=left] node {{\scriptsize $\lambda_H (1 - (1 - p_H^2)^{h})$} \\ {\scriptsize $+ \lambda_E (1 - (1 - p_E p_H)^{h})$}} (l)
		(l) edge[bend right, dashed] node {} (s)
		(s) edge[bend right, auto=right] node {\scriptsize $\lambda_E (1 - p_E p_H)^{h} (1 - p_E^2)^{e}$} (t)
		(t) edge[bend right, dashed] node {} (s)
		(s) edge[bend right, auto=right] node {{\scriptsize $\lambda_H (1 - p_H^2)^{h} (1 - (1 - p_E p_H)^{e}) $} \\ {\scriptsize $+ \lambda_E (1 - p_E p_H)^{h} (1 - (1 - p_E^2)^{e})$}} (b)
		(b) edge[bend right, dashed] node {} (s)
		(b) edge[bend right, dashed] node {} (br)
		(br) edge[bend right, dashed] node {} (b)
		(b) edge[bend right, dashed] node {} (bl)
		(bl) edge[bend right, dashed] node {} (b)
		(t) edge[bend right, dashed] node {} (tr)
		(tr) edge[bend right, dashed] node {} (t)
		(t) edge[bend right, dashed] node {} (tl)
		(tl) edge[bend right, dashed] node {} (t)
		(r) edge[bend right, dashed] node {} (br)
		(br) edge[bend right, dashed] node {} (r)
		(l) edge[bend right, dashed] node {} (bl)
		(bl) edge[bend right, dashed] node {} (l)
		(r) edge[bend right, dashed] node {} (tr)
		(tr) edge[bend right, dashed] node {} (r)
		(l) edge[bend right, dashed] node {} (tl)
		(tl) edge[bend right, dashed] node {} (l);

\end{tikzpicture}
\caption{CTMC underlying the market under $\BH$ policy. Transition rates are given only for solid arrows. }
\label{fig:2d:walk}
\end{figure}


We further remark that as the above transition rates indicate the only possible transition from state $[h,e]$ is to its neighbors (i.e, state $[h',e']$ such that  $ \mid h' - h \mid  + \mid e' - e \mid = 1.$), and therefore the process is a $2$-dimensional continuous-time spatially non-homogenous random walk. Figure \ref{fig:2d:walk} illustrates this random walk along with its transition rates.
Lastly, we note that both the rightward and downward rates \eqref{eq:transtion:2} and \eqref{eq:transtion:4} depend on the  priority set by the policy. As we will see in the next subsection, these rates will be different when priorities are given to $E$ agents rather than $H$ ones.
However, once the priority is set, the tie breaking among the same type agents does not impact the transition rates.
In \textit{ BilateralMatch(H)} Policy, we assumes such ties are broken at random, however, our result also holds for modified version of the policy
that employ other tie breaking rules {\em within} each type, for instance, in favor of the longest waiting agent.


In Appendix \ref{app:existence_proofs}, we prove that the above CTMC is positive recurrent, and therefore reaches steady-state. This is fairly intuitive given the above transition rates and the   ``self-regulating'' behavior of the process. If the market becomes ``too large'' the probability that an arriving agent can form a $2$-way increases; on the other hand, if the market becomes ``too small'' the probability that an arriving agent can form a $2$-way decreases. In what follows, we analyze the chain in steady state. In particular, in steady state, the expected drift in both horizontal and vertical dimension is zero. Conditioned on $[H_t^{\BH},  E_t^{\BH}] = [h,e]$ the drifts are given in \eqref{eq:transtion:1}-\eqref{eq:transtion:4}, and therefore,


\begin{subequations}
\begin{align}
& \E\left[\lambda_H (1 - p_H^2)^{h} (1 - p_E p_H)^{e}  - \lambda_H (1 - (1 - p_H^2)^{h}) - \lambda_E (1 - (1 - p_E p_H)^{h})\right] = 0  \label{eq:approx1}\\
& \E\left[\lambda_E (1 - p_E p_H)^{h} (1 - p_E^2)^{e}  -  \lambda_H(1 - p_H^2)^{h} (1 - (1 - p_E p_H)^{e}) - \lambda_E (1 - p_E p_H)^{h} (1 - (1 - p_E^2)^{e}) \right] = 0 \label{eq:approx2}
\end{align}
\end{subequations}

If we move the expectation inside the functions, and solve  the above system of nonlinear equations, it provides us with an approximation of $\E[H^{\BH}]$ and $\E[E^{\BH}]$.
In fact, some algebra shows:

\begin{itemize}
\item[-] For the case $\lambda_H < \lambda_E$, if we plug in $\left[\frac{\ln \left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right)}{p_E p_H}, \frac{-\ln (2)}{\ln (1-p_E^2 )} \right]$ into \eqref{eq:approx1},  the right-hand side will be an $o(p_H)$ term.
\item[-] For the case, $\lambda_H > \lambda_E$, if we plug in $\left[\frac{\ln \left( \frac{2 \lambda_H}{\lambda_H + \lambda_E} \right)}{p_H^2}, 0 \right]$  into \eqref{eq:approx2},  the right-hand side will be an $o(p_H)$ term.
\end{itemize}

Even though the above argument is just a heuristic, it indeed gives us the correct value of $\E[H^{\BH}]$ in both cases. 
In order to precisely calculate $\E[H^{\BH}]$ and prove Theorem \ref{th:bilat_prioH}, in the following two propositions we show that $H^{\BH}$ is indeed highly concentrated 
around its mean:

%The proof of Theorem \ref{th:bilat_prioH} relies on the following concentration results:

\begin{restatable}{proposition}{propUpperHprioH}\emph{[Upper-bound]}
\label{prop:upper_H_prio_H}
Under $\BH$ and in steady-state,  
\begin{itemize}
\item[-] If $\lambda_H < \lambda_E$, there exists a constant $c_2>0$ such that:
$$ \P\left[H^\BH \geq \frac{1}{p_E p_H} \left( \ln\left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right) + c_2 p_H^{1/4} \right) \right]  \leq o(\sqrt{p_H}).$$
%Where $\gamma(p_H) =  \frac{\lambda_H}{\lambda_E - (\lambda_E - \lambda_H)e^{- \xi(p_H)}} + O(p_H)$.
\item[-] If $\lambda_H > \lambda_E$, there exists a constant $c_1>0$ such that:
$$ \P\left[H^\BH \geq \frac{1}{p_H^2} \left( \ln\left(\frac{2 \lambda_H}{\lambda_E + \lambda_H}\right) + c_1 p_H^{1/2} \right) \right]  \leq o(\sqrt{p_H}).$$
%Where $\gamma(p_H) = \frac{ e^{- \xi(p_H)} }{ 2 -  e^{- \xi(p_H)}} +O(p_H^2) $.
\end{itemize}
\end{restatable}


\begin{restatable}{proposition}{propLowerHprioH}\emph{[Lower-bound]}
\label{prop:lower_H_prio_H}
Under $\BH$ and in steady-state,
%\begin{itemize}
%\item[-] If $\lambda_H < \lambda_E$, then $\E[H] \geq \frac{\ln\left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right)}{p_E p_H} + o\left( \frac{1}{p_H} \right)$.
%\item[-] If $\lambda_H > \lambda_E$, then $\E[H] \geq \frac{\ln\left(\frac{2 \lambda_H}{\lambda_H + \lambda_E} \right)}{p_H^2} + o \left( \frac{1}{p_H^2} \right)$.
%\end{itemize}
\begin{itemize}
\item[-] If $\lambda_H < \lambda_E$, then there exists a constant $c_3$ such that:
$$ \P\left[H^\BH \leq \frac{\ln\left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right)}{p_E p_H} - c_3 p_H^{-3/4} \right]  \leq  o(\sqrt{p_H}).$$%\frac{2\eta \cdot o(p_H^4) }{f(\eta) - g(\eta+1)}  + \frac{\gamma(p_H)^k}{1 -\gamma(p_H)}.$$
%Where $\gamma(p_H) = 1 - p_H^{1/4} + o(p_H^{1/4})$.
\item[-] If $\lambda_H > \lambda_E$, then  there exists a constant $c_4$ such that:
$$ \P\left[H^\BH \leq \frac{\ln{2 \theta}}{p_H^2} - c_4 p_H^{-3/2} \right]  \leq  o(p_H).$$% \frac{2\eta \cdot o(p_H^4)} {f(\eta) - g(\eta+1)}  + \frac{\gamma(p_H)^k}{1 - \gamma(p_H)}.$$
%Where $\gamma(p_H) =  1 - p_H^{1/2} + o(p_H^{1/2})$.
\end{itemize}
\end{restatable}


Proof of Theorem \ref{th:bilat_prioH} is a straightforward application of the above propositions. The details are presented in Appendix \ref{subsec:proof:thm1}. The proof of both propositions are deferred to Appendix \ref{app:bilat_prioH}.

\vm{edited here.}

%\begin{proof}[Proof of Theorem \ref{th:bilat_prioH}]
%We first upper-bound  $\E[H^\BH] $ using Proposition \ref{prop:upper_H_prio_H}: Let
%\begin{equation}
%v(\lambda_H, \lambda_E, p_E, p_H) = \Bigg\{
%\label{eq:2d-walk}
%\begin{matrix}
%& \frac{1}{p_H^2} \left( \ln\left(\frac{2 \lambda_H}{\lambda_E + \lambda_H}\right) + \xi(p_H) \right) + p_H^{-3/4} &\text{ when } \lambda_H < \lambda_E, \\
%&\frac{1}{p_E p_H} \left( \ln\left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right) + \xi(p_H) \right) + p_H^{-3/4} &\text{ when } \lambda_H > \lambda_E.
%\end{matrix}
%\end{equation}
%
%Using the equality  $\E[H^{\BH}] = \sum_{i = 0}^{\infty} \P[H^{\BH} \geq i]$, we have:
%\begin{equation}
%\begin{split}
%\E[H^{\BH}] &= \sum_{i = 0}^{v(\lambda_H, \lambda_E, p_E, p_H)} \P[H \geq i] +  \sum_{i = v(\lambda_H, \lambda_E, p_E, p_H)}^{\infty} \P[H \geq i]\\
%&\leq v(\lambda_H, \lambda_E, p_E, p_H) + \sum_{i = p_H^{-3/4}}^{\infty} \frac{\gamma(p_H)^i}{1- \gamma(p_H)} \\
%& \leq  v(\lambda_H, \lambda_E, p_E, p_H) + \frac{\gamma(p_H)^{p_H^{-3/4}}}{(1- \gamma(p_H))^2}.
%\end{split}
%\end{equation}
%\vm{Max: please fix the $\xi(p_H)$. Also  why $i = p_H^{-3/4}$ is the second sum above? }
%
%
%Applying Fact \ref{cl:dl}, and some algebra we get the following upper-bound on $\E[H^\BH]$:
%\begin{itemize}
%\item[-] If $\lambda_H < \lambda_E$, then $\E[H^\BH] \leq \frac{\ln\left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right)}{p_E p_H} + o\left( \frac{1}{p_H} \right)$.
%\item[-] If $\lambda_H > \lambda_E$, then $\E[H^\BH] \leq \frac{\ln\left(\frac{2 \lambda_H}{\lambda_H + \lambda_E} \right)}{p_H^2} + o \left( \frac{1}{p_H^2} \right)$.
%\end{itemize}
%Now we proceed to lower-bound  $\E[H^\BH] $: Applying Markov inequality to $\E[H^\BH] $ and  using Proposition \ref{prop:lower_H_prio_H}, we get the following lower-bound on $\E[H^\BH]$:
%
%%First we note that for any $\eta \in \R$: $\E[X] \geq \eta \P[X > \eta]$. Applying this inequality to $\E[H^\BH] $ and  using Proposition \ref{prop:lower_H_prio_H}, we get the following lower-bound on $\E[H^\BH]$:
%\begin{itemize}
%\item[-] If $\lambda_H < \lambda_E$, then $\E[H^\BH] \geq \frac{\ln\left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right)}{p_E p_H} + o\left( \frac{1}{p_H} \right)$.
%\item[-] If $\lambda_H > \lambda_E$, then $\E[H^\BH] \geq \frac{\ln\left(\frac{2 \lambda_H}{\lambda_H + \lambda_E} \right)}{p_H^2} + o \left( \frac{1}{p_H^2} \right)$.
%\end{itemize}
%This completes the proof.
%\end{proof}




%
%\begin{corollary}
%\label{cor:upper_H}
%Under $\BH$,
%\begin{itemize}
%\item[-] If $\lambda_H < \lambda_E$, then $\E[H^\BH] \leq \frac{\ln\left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right)}{p_E p_H} + o\left( \frac{1}{p_H} \right)$.
%\item[-] If $\lambda_H > \lambda_E$, then $\E[H^\BH] \leq \frac{\ln\left(\frac{2 \lambda_H}{\lambda_H + \lambda_E} \right)}{p_H^2} + o \left( \frac{1}{p_H^2} \right)$.
%\end{itemize}
%\end{corollary}
%
%\begin{proof}
%Let  $\xi(p_H) = \sqrt{p_H}$. In both cases there exists a constant $c > 0$ such that $\gamma(p_H) = 1 - c\sqrt{p_H}$. Furthermore, let
%
%\begin{equation}
%v(\lambda_H, \lambda_E, p_E, p_H) = \Bigg\{
%\label{eq:2d-walk}
%\begin{matrix}
%& \frac{1}{p_H^2} \left( \ln\left(\frac{2 \lambda_H}{\lambda_E + \lambda_H}\right) + \xi(p_H) \right) + p_H^{-3/4} &\text{ when } \lambda_H < \lambda_E, \\
%&\frac{1}{p_E p_H} \left( \ln\left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right) + \xi(p_H) \right) + p_H^{-3/4} &\text{ when } \lambda_H > \lambda_E.
%\end{matrix}
%\end{equation}
%
%
%From Proposition \ref{prop:upper_H_prio_H}, we get:
%\begin{equation}
%\begin{split}
%\E[H] &= \sum_{i = 0}^{v(\lambda_H, \lambda_E, p_E, p_H)} \P[H \geq i] +  \sum_{i = v(\lambda_H, \lambda_E, p_E, p_H)}^{\infty} \P[H \geq i]\\
%&\leq v(\lambda_H, \lambda_E, p_E, p_H) + \sum_{i = p_H^{-3/4}}^{\infty} \frac{\gamma(p_H)^i}{1- \gamma(p_H)} \\
%& \leq  v(\lambda_H, \lambda_E, p_E, p_H) + \frac{\gamma(p_H)^{p_H^{-3/4}}}{(1- \gamma(p_H))^2}
%\end{split}
%\end{equation}
%We can conclude using Claim \ref{cl:dl}.
%\end{proof}
%
%\begin{restatable}{proposition}{propLowerHprioH}
%\label{prop:lower_H_prio_H}
%Under $\BH$ and in steady-state,
%%\begin{itemize}
%%\item[-] If $\lambda_H < \lambda_E$, then $\E[H] \geq \frac{\ln\left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right)}{p_E p_H} + o\left( \frac{1}{p_H} \right)$.
%%\item[-] If $\lambda_H > \lambda_E$, then $\E[H] \geq \frac{\ln\left(\frac{2 \lambda_H}{\lambda_H + \lambda_E} \right)}{p_H^2} + o \left( \frac{1}{p_H^2} \right)$.
%%\end{itemize}
%\begin{itemize}
%\item[-] If $\lambda_H < \lambda_E$, then there exists a constant $c_3$ such that:
%$$ \P\left[H^\BH \leq \frac{\ln\left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right)}{p_E p_H} - c_3 p_H^{-3/4} \right]  \leq  o(\sqrt{p_H}).$$%\frac{2\eta \cdot o(p_H^4) }{f(\eta) - g(\eta+1)}  + \frac{\gamma(p_H)^k}{1 -\gamma(p_H)}.$$
%%Where $\gamma(p_H) = 1 - p_H^{1/4} + o(p_H^{1/4})$.
%\item[-] If $\lambda_H > \lambda_E$, then  there exists a constant $c_4$ such that:
%$$ \P\left[H^\BH \leq \frac{\ln{2 \theta}}{p_H^2} - c_4 p_H^{-3/2} \right]  \leq  o(p_H).$$% \frac{2\eta \cdot o(p_H^4)} {f(\eta) - g(\eta+1)}  + \frac{\gamma(p_H)^k}{1 - \gamma(p_H)}.$$
%%Where $\gamma(p_H) =  1 - p_H^{1/2} + o(p_H^{1/2})$.
%\end{itemize}
%\end{restatable}
%The proof is deferred to Appendix \ref{app:bilat_prioH}.
%\begin{corollary}
%\label{cor:lower_H_prio_H}
%Under $\BH$,
%\begin{itemize}
%\item[-] If $\lambda_H < \lambda_E$, then $\E[H^\BH] \geq \frac{\ln\left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right)}{p_E p_H} + o\left( \frac{1}{p_H} \right)$.
%\item[-] If $\lambda_H > \lambda_E$, then $\E[H^\BH] \geq \frac{\ln\left(\frac{2 \lambda_H}{\lambda_H + \lambda_E} \right)}{p_H^2} + o \left( \frac{1}{p_H^2} \right)$.
%\end{itemize}
%\end{corollary}
%
%\begin{proof}
%This is a direct consequence of the following fact for any $\eta \in \R$: $\E[X] \geq \eta \P[X > \eta]$.
%\end{proof}
%%
%%
%%
%%If $\lambda_H > \lambda_E$, $\left(\frac{\ln \left( \frac{2 \lambda_H}{\lambda_H + \lambda_E} \right)}{p_H^2}, 0 \right)$ is a solution to (\ref{eq:transitions_mean_field}) up to a $o(p_H)$ term.
%%
%%If $\lambda_H < \lambda_E$, $\left(\frac{\ln \left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right)}{p_E p_H}, \frac{-\ln (2)}{\ln (1-p_E^2 )} \right)$ is a solution to (\ref{eq:transitions_mean_field}) up to a $o(p_H)$ term.
%%
%%
%%
%%Having  the transition rate of the random walk, we observe that both the leftward and the upward rates are exponentially decreasing in the number of agents $[h,e]$. This implies an intuitive ``self-regulating'' behavior of the process.
%%
%%vertices in the graph can be described as a continuous time random walk $(H(t), E(t)) \in \Z^2$ with rate matrix satisfying:
%%
%%
%%
%%\begin{restatable}{claim}{claimBilatHSS}
%%\label{cl:existence_bilat_H}
%%Under $\BH$, the evolution of the numbers of $H$ and $E$ vertices in the graph can be described as a continuous time random walk $(H(t), E(t)) \in \N^2$ with rate matrix satisfying:
%%\begin{equation}
%%\label{eq:transitions}
%%\begin{split}
%%Q([h,e],[h+1,e]) &= \lambda_H (1 - p_H^2)^{h} (1 - p_E p_H)^{e}\\
%%Q([h,e],[h-1,e]) &=  \lambda_H (1 - (1 - p_H^2)^{h}) + \lambda_E (1 - (1 - p_E p_H)^{h})\\
%%Q([h,e],[h,e + 1])&=\lambda_E (1 - p_E p_H)^{h} (1 - p_E^2)^{e}\\
%%Q([h,e],[h,e-1])&= \lambda_H (1 - p_H^2)^{h} (1 - (1 - p_E p_H)^{e}) + \lambda_E (1 - p_E p_H)^{h} (1 - (1 - p_E^2)^{e}))
%%\end{split}
%%\end{equation}
%%Furthermore, $(H(t), E(t))$ is positive recurrent.%\footnote{\mb{Reference to a Foster-like result for jump processes ?}}
%%\end{restatable}
%%The proof is deferred to Appendix \ref{app:existence_proofs}.
%%We will denote by $(H, E)$ the random variables sampled from the resulting steady-state distribution.
%%
%%
%%
%%%\subsubsection{Priority to H}
%%%When priorities are given to $H$ agents, the numbers $(N^H_t, N^E_t)_{t \geq 0}$ of nodes in the system follows a markov chain of the form (\ref{eq:transitions}) with transitions:
%%
%%\bilatprioH*
%%
%%An intuitive explanation can be obtained by the following heuristic: at equilibrium, the number of $H$ ($E$) vertices have equal probability of increasing and decreasing. This yields the following system of two equations:
%%\begin{equation}
%%\label{eq:transitions_mean_field}
%%\begin{split}
%%\lambda_H (1 - p_H^2)^{h} (1 - p_E p_H)^{e} &= \lambda_H (1 - (1 - p_H^2)^{h}) + \lambda_E (1 - (1 - p_E p_H)^{h})  \\
%%\lambda_E (1 - p_E p_H)^{h} (1 - p_E^2)^{e} &= \lambda_H(1 - p_H^2)^{h} (1 - (1 - p_E p_H)^{e}) + \lambda_E (1 - p_E p_H)^{h} (1 - (1 - p_E^2)^{e}))  \\
%%\end{split}
%%\end{equation}
%%
%%If $\lambda_H > \lambda_E$, $\left(\frac{\ln \left( \frac{2 \lambda_H}{\lambda_H + \lambda_E} \right)}{p_H^2}, 0 \right)$ is a solution to (\ref{eq:transitions_mean_field}) up to a $o(p_H)$ term.
%%
%%If $\lambda_H < \lambda_E$, $\left(\frac{\ln \left(\frac{\lambda_E}{\lambda_E - \lambda_H}\right)}{p_E p_H}, \frac{-\ln (2)}{\ln (1-p_E^2 )} \right)$ is a solution to (\ref{eq:transitions_mean_field}) up to a $o(p_H)$ term.
%%
%%\begin{proof}[Proof idea]
%%The proof of Theorem \ref{th:bilat_prioH} is given in appendix \ref{app:bilat_prioH}. The idea is that if we are able to bound the transition probabilities, then Lemmas \ref{lem:lower_bound} and \ref{lem:upper_bound} provide us with concentration bounds on the left and right tail probabilities. From these bounds we can then find bounds on the expected number of $H$ vertices.
%%\end{proof}
%%
%%\subsection{Proof idea of Theorem \ref{th:bilat_prioE}}
%%\begin{restatable}{claim}{claimBilatESS}
%%Under $\BE$, the evolution of the numbers of $H$ and $E$ vertices follows a continuous time random walk $(H(t), E(t)) \in \N^2$ with rate matrix satisfying:
%%\begin{equation}
%%\label{eq:transitions}
%%\begin{split}
%%Q([h,e],[h+1,e]) &= \lambda_H (1 - p_H^2)^{h} (1 - p_E p_H)^{e}\\
%%Q([h,e],[h-1,e]) &=  \lambda_H (1 - p_E p_H)^{e}(1 - (1 - p_H^2)^{h}) + \lambda_E (1 - p_E^2)^{e}(1 - (1 - p_E p_H)^{h}) \\
%%Q([h,e],[h,e + 1])&=\lambda_E (1 - p_E p_H)^{h} (1 - p_E^2)^{e} \\
%%Q([h,e],[h,e-1])&= \lambda_H (1 - (1 - p_E p_H)^{e}) + \lambda_E (1 - (1 - p_E^2)^{e}))
%%\end{split}
%%\end{equation}
%%Furthermore, $(H(t), E(t))$ is aperiodic and positive recurrent.
%%\end{restatable}
%%The proof is deferred to Appendix \ref{app:existence_proofs}.
%%We will denote by $(H, E)$ the random variables sampled from the resulting steady-state distribution.
%%
%%An intuitive explanation can be obtained by the following heuristic: at equilibrium, the number of $H$ ($E$) vertices have equal probability of increasing and decreasing. This yields the following system of two equations:
%%\begin{equation}
%%\label{eq:transitions_mean_field}
%%\begin{split}
%%\lambda_H (1 - p_H^2)^{h} (1 - p_E p_H)^{e} &=  \lambda_H (1 - p_E p_H)^{e}(1 - (1 - p_H^2)^{h}) + \lambda_E (1 - p_E^2)^{e}(1 - (1 - p_E p_H)^{h})  \\
%%\lambda_E (1 - p_E p_H)^{h} (1 - p_E^2)^{e} &=  \lambda_H (1 - (1 - p_E p_H)^{e}) + \lambda_E (1 - (1 - p_E^2)^{e}))  \\
%%\end{split}
%%\end{equation}
%%
%%If $\lambda_H > \lambda_E$, $\left(\frac{\ln \left( \frac{2 \lambda_H}{\lambda_H + \lambda_E} \right)}{p_H^2}, 0 \right)$ is a solution to (\ref{eq:transitions_mean_field}) up to a $o(p_H)$ term.
%%
%%If $\lambda_H < \lambda_E$, $\left(\frac{\ln \left(\frac{\lambda_E + \lambda_H}{\lambda_E - \lambda_H}\right)}{p_E p_H}, \frac{\ln \left( \frac{\lambda_E + \lambda_H}{2 \lambda_E}\right)}{\ln (1-p_E^2 )} \right)$ is a solution to (\ref{eq:transitions_mean_field}) up to a $o(p_H)$ term.
%%

